Autonomous Intraluminal Navigation of a Soft Robot using Deep-Learning-based Visual Servoing

Navigation inside luminal organs is an arduous task that requires non-intuitive coordination between the movement of the operator's hand and the information obtained from the endoscopic video. The development of tools to automate certain tasks could alleviate the physical and mental load of doctors during interventions, allowing them to focus on diagnosis and decision-making tasks. In this paper, we present a synergic solution for intraluminal navigation consisting of a 3D printed endoscopic soft robot that can move safely inside luminal structures. Visual servoing, based on Convolutional Neural Networks (CNNs) is used to achieve the autonomous navigation task. The CNN is trained with phantoms and in-vivo data to segment the lumen, and a model-less approach is presented to control the movement in constrained environments. The proposed robot is validated in anatomical phantoms in different path configurations. We analyze the movement of the robot using different metrics such as task completion time, smoothness, error in the steady-state, and mean and maximum error. We show that our method is suitable to navigate safely in hollow environments and conditions which are different than the ones the network was originally trained on.

==> table_notuse.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\caption{Results of the Intra-Luminal Navigation task}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
    & \multicolumn{2}{c}{SL} & \multicolumn{2}{c}{RC} & \multicolumn{2}{c}{LC} & \multicolumn{2}{c}{SC} \\ \hline
    & Avg        & Std       & Avg         & Std      & Avg         & Std      & Avg        & Std       \\ \hline
CT  & 81,24      & 7,28      & 119,73      & 33,59    & 157,52      & 54,77    & 212,9      & 57,89     \\
ME  & 0,86       & 0,33      & 2,17        & 0,34     & 1,74        & 0,32     & 1,99       & 0,29      \\
MxE & 2,09       & 0,23      & 6,11        & 0,37     & 5,12        & 0,56     & 4,35       & 0,41      \\
AUC & 412,76     & 170,48    & 1456,59     & 469,9    & 1467,38     & 479,4    & 2262,87    & 709,28    \\
LDJ & -12,54     & 0,4       & -13,52      & 1,42     & -14,49      & 1,41     & -15,32     & 1,1       \\
SAL & -9,16      & 0,15      & -9,16       & 0,27     & -9,48       & 0,37     & -9,8       & 0,34      \\
NP  & 105,25     & 14,97     & 130,8       & 42,31    & 160,6       & 1,41     & 169,13     & 40,79     \\ \hline
\end{tabular}%
}
\end{table}

\begin{table}[]
\caption{Results of the Intra-Luminal Navigation task2}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline
    & SL                         & RC                         & LC                         & SV                         \\ \hline
CT  & 81,24      $\pm$ 7,28      & 119,73      $\pm$ 33,59    & 157,52      $\pm$ 54,77    & 212,90     $\pm$ 57,89     \\
ME  & 0,86       $\pm$ 0,33      & 2,17        $\pm$ 0,34     & 1,74        $\pm$ 0,32     & 1,99       $\pm$ 0,29      \\
MxE & 2,09       $\pm$ 0,23      & 6,11        $\pm$ 0,37     & 5,12        $\pm$ 0,56     & 4,35       $\pm$ 0,41      \\
AUC & 412,76     $\pm$ 170,48    & 1456,59     $\pm$ 469,90   & 1467,38     $\pm$ 479,4    & 2262,87    $\pm$ 709,28    \\
LDJ & -12,54     $\pm$ 0,40      & -13,52      $\pm$ 1,42     & -14,49      $\pm$ 1,41     & -15,32     $\pm$ 1,10      \\
SAL & -9,16      $\pm$ 0,15      & -9,16       $\pm$ 0,27     & -9,48       $\pm$ 0,37     & -9,80      $\pm$ 0,34      \\
NP  & 105,25     $\pm$ 14,97     & 130,80      $\pm$ 42,31    & 160,60      $\pm$ 1,41     & 169,13     $\pm$ 40,79     \\ \hline
\end{tabular}%
}
\end{table}


\begin{table}
    \centering    
    \caption{Completion time in different paths}
    \label{table:completion_time}
    \begin{tabular}{cccc}
    \hline
    Path ID & \multicolumn{2}{c}{Avg.(s) $\pm$ STD} & p-value \\
            & Jac & P. Field & \\ 
    1 & 111.87 $\pm$ 31.28 & 81.24 $\pm$ 7.28  & $<0.05$\\
    2 & 163.07 $\pm$ 59.03 & 119.73 $\pm$ 33.59 & 0.05\\
    3 & 194.47 $\pm$ 50.61 & 157.52 $\pm$ 54.77 & $<0.05$ \\
    4 & 229.95 $\pm$ 38.45 & 212.90 $\pm$ 57.89 & $<0.05$ \\
    \hline
    \end{tabular}

\end{table}

\begin{table}
    \centering    
    \caption{Smoothness: log dimensionless jerk}
    \label{table:smooth_logdimjerk}
    \begin{tabular}{cccc}
    \hline
    Path ID & \multicolumn{2}{c}{Avg. $\pm$ STD} & p-value \\
            & Jac & P. Field & \\ 
    1 &  -13.43 $\pm$ 1.05 & -12.54 $\pm$ 0.40  & $<0.05$\\
    2 & -14.35  $\pm$ 1.4 & -13.52 $\pm$ 1.42 & $<0.05$ \\
    3 & -15.22 $\pm$ 1.12 & -14.49 $\pm$ 1.41 & $<0.05$ \\
    4 & -15.45 $\pm$ 0.70 & -15.32 $\pm$ 1.10 & $<0.05$ \\
    \hline
    \end{tabular}
\end{table}

\begin{table}
    \centering    
    \caption{Smoothness: spectral arc-length}
    \label{table:smooth_sparc}
    \begin{tabular}{cccc}
    \hline
    Path ID & \multicolumn{2}{c}{Avg. $\pm$ STD} & p-value \\
            & Jac & P. Field & \\ 
    1 & -9.52 $\pm$ 0.36 & -9.16 $\pm$ 0.15 & $<0.05$\\
    2 & -9.48 $\pm$ 0.34 & -9.16 $\pm$ 0.27 & 0.05 \\
    3 & -9.73 $\pm$ 0.32 & -9.48 $\pm$ 0.37 & $<0.05$ \\
    4 & -9.91 $\pm$ 0.18 & -9.80 $\pm$ 0.34 & $<0.05$ \\
    \hline
    \end{tabular}
\end{table}

\begin{table}
    \centering    
    \caption{Smoothness:Number of peaks}
    \label{table:smooth_num_peaks}
    \begin{tabular}{cccc}
    \hline
    Path ID & \multicolumn{2}{c}{Avg. $\pm$ STD} & p-value \\
            & Jac & P. Field & \\ 
    1 &  135.25 $\pm$ 37.69 & 105.25 $\pm$ 14.97 & $<0.05$\\
    2 & 174.13 $\pm$ 69.04 & 130.80 $\pm$ 42.31 & $<0.05$\\
    3 & 198.93 $\pm$ 49.72 & 160.60 $\pm$ 1.41 & $<0.05$ \\
    4 & 180.13 $\pm$ 41.24 & 169.13 $\pm$ 40.79 & $<0.05$ \\
    \hline
    \end{tabular}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
        Path ID & Metric & MEAN & MEDIAN & STDV \\ \hline
        1 & AUC & 412.75750000000016 & 446.12750000000017 & 170.47723002280978 \\
& Max Error & 2.0874999999999986 & 2.115000000000002 &  0.23252688016657472 \\
& Mean Error & 0.8557962466978226 & 0.9201280931896593 &  0.33201058432791974 \\ \hline
2 & AUC & 1456.5923228666502 & 1363.1628879105556 &  469.8946298424848 \\
& Max Eerror & 6.106777375693041 & 6.22508417316547 & 0.3434007566779139\\
& Mean Error & 2.1680855230397595 & 2.115124658347321 &  0.37162623718707966\\ \hline
3 & AUC & 1467.3275676653982 & 1342.56703326584 &  479.3950027806724 \\
& Max Error & 5.120645650047976 & 4.8688922517300455 &  0.55949421479747 \\
& Mean Error & 1.7403764350592688 & 1.6047230955279101 &  0.31591793140216223 \\ \hline
4 & AUC & 2262.8737932929457 & 2535.185292553057 &  709.2785535576372 \\ 
& Max Error & 4.35062112714395 & 4.2282850645031544 & 0.4098033263783747 \\
& Mean Error & 1.993969334732172 & 1.9946403601113236 &  0.29184773277858506 \\


    \end{tabular}
    \caption{EDIT TABLE}
    \label{tab:my_label}
\end{table}


\begin{table*}[tbp]
\caption{Results of the IntraLuminal Navigation task for the 4 different path scenarios.}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Completion time (s)} & \multicolumn{1}{c}{Mean absolute error (mm)}  & \multicolumn{1}{c}{Max absolute error (mm)} & \multicolumn{1}{c}{Area under curve (mm$^2$)} & \multicolumn{1}{c}{Log-dimensionless jerk}  & \multicolumn{1}{c}{Spectral arc-length}        & \multicolumn{1}{c}{Number of peaks}           \\ \hline
$A$  & 81.2 $\pm$7.2  & 0.86$\pm$0.33 & 2.09$\pm$0.23 & 412.7$\pm$170  & -12.54$\pm$0.40 & -9.16$\pm$0.15 & 105.2$\pm$14.9 \\
$B$  & 119.7$\pm$33.5 & 2.17$\pm$0.34 & 6.11$\pm$0.37 & 1456.5$\pm$469 & -13.52$\pm$1.42 & -9.16$\pm$0.27 & 130.8$\pm$42.8  \\
$C$  & 157.5$\pm$57.7 & 1.74$\pm$0.32 & 5.12$\pm$0.56 & 1467.3$\pm$479 & -14.49$\pm$1.41 & -9.48$\pm$0.37 & 160.6$\pm$1.41  \\
$D$  & 212.9$\pm$57.8  & 1.99$\pm$0.29 & 4.35$\pm$0.41 & 2262.8$\pm$709 & -15.32$\pm$1.10 & -9.80$\pm$0.34  & 169.1$\pm$40.7  \\ \hline

\end{tabular}%
}
\end{table*}

%from 1020.2021
\begin{table}[tbp]
\scriptsize
\caption{
\scriptsize
Results of the intraluminal navigation task for the 4 different paths.}
\centering
%\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{ccccc}
     & Path $A$ & Path $B$ & Path $C$ & Path $D$ \\
\hline
Metrics*   & Avg $\pm$ STD  & Avg $\pm$ STD  & Avg $\pm$ STD  & Avg $\pm$ STD \\ 
\hline
CT (s)     & 81.2 $\pm$7.2  & 119.7$\pm$33.5 & 157.5$\pm$57.7 & 212.9$\pm$57.8 \\
MAE (mm)   & 0.86$\pm$0.33  & 2.17$\pm$0.34  & 1.74$\pm$0.32  & 1.99$\pm$0.29  \\
MaxAE (mm) & 2.09$\pm$0.23  & 6.11$\pm$0.37  & 5.12$\pm$0.56  & 4.35$\pm$0.41  \\
LDJ        & -12.5$\pm$0.40 & -13.5$\pm$1.42 & -14.4$\pm$1.41 & -15.3$\pm$1.10 \\
SPARC      & -9.16$\pm$0.15 & -9.16$\pm$0.27 & -9.48$\pm$0.37 & -9.80$\pm$0.34 \\ 
NP         & 105.2$\pm$14.9 & 130.8$\pm$42.8 & 163.06$\pm$58.4& 169.10$\pm$40.70 \\ \hline
\multicolumn{5}{l}{\scriptsize{*Metrics: Completion Time (CT), Mean Absolute Error (MAE), Max Absolute}}\\
\multicolumn{5}{l}{\scriptsize{Error (MaxAE), Log-dimensionless Jerk (LDJ), Spectral Arc Length (SPARC)}}\\
\multicolumn{5}{l}{\scriptsize{and number of peaks (NP).}}
\end{tabular}%
\end{table}
